On Wyner's Common Information in the Gaussian Case

Wyner's Common Information and a natural relaxation are studied in the special case of Gaussian random variables. The relaxation replaces conditional independence by a bound on the conditional mutual information. The main contribution is the proof that Gaussian auxiliaries are optimal, leading to a closed-form formula. As a corollary, the proof technique also establishes the optimality of Gaussian auxiliaries for the Gaussian Gray-Wyner network, a long-standing open problem.

==> gray_wyner.tex <==

%
\begin{tikzpicture}
\draw[->, line width=1pt](0,0)--(9,0);
\draw[->, line width=1pt](0,0)--(0,6.5);
\draw[black,thick,anchor=north] (8.5,0) node{$De^{\beta}$};
\draw[black,thick,anchor=center] (0,7) node{$\mathrm{R}_{D,\beta}(X,Y)$};
\pgfplotsset{ticks=none}
\begin{axis}[%
hide y axis,
hide x axis,
width=4in,
height=3in,
xmin=0,
xmax=1,
ymin=0,
ymax=4.5,
xlabel={$\gamma_i$},
ylabel={$C_{\gamma_i}({\ve X}_i,{\ve Y}_i)$},
legend style={at={(0.8,0.8)}, legend cell align=center, align=center, draw=white!15!black}
]
\addplot [line width=1pt, draw=none, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
0.5	0.549306144334055\\
0.51	0.529695787757414\\
0.52	0.510825623765991\\
0.53	0.492641801680553\\
0.54	0.475096141774918\\
0.55	0.458145365937077\\
0.56	0.441750454525582\\
0.57	0.425876105368292\\
0.58	0.410490276034915\\
0.59	0.395563794460075\\
0.6	0.381070026023448\\
0.61	0.3669845875401\\
0.62	0.353285100446043\\
0.63	0.339950976904962\\
0.64	0.326963233703332\\
0.65	0.314304329711187\\
0.66	0.301958023416001\\
0.67	0.289909247626471\\
0.68	0.278143998921374\\
0.69	0.266649239809025\\
0.7	0.255412811882995\\
0.71	0.244423358523608\\
0.72	0.233670255913126\\
0.73	0.22314355131421\\
0.74	0.212833907712842\\
0.75	0.202732554054082\\
0.76	0.192831240405992\\
0.77	0.183122197477442\\
0.78	0.173598099992094\\
0.79	0.164252033486018\\
0.8	0.15507746415192\\
0.81	0.146068211400581\\
0.82	0.13721842285088\\
0.83	0.128522551494945\\
0.84	0.119975334815296\\
0.85	0.111571775657105\\
0.86	0.1033071246815\\
0.87	0.0951768642456094\\
0.88	0.087176693572389\\
0.89	0.0793025150883192\\
0.9	0.0715504218203367\\
0.91	0.0639166857549423\\
0.92	0.0563977470726723\\
0.93	0.0489902041801019\\
0.94	0.0416908044695256\\
0.95	0.0344964357434758\\
0.96	0.0274041182474975\\
0.97	0.0204109972601276\\
0.98	0.0135143361939597\\
0.99	0.00671151016607036\\
1	0\\
};
\addlegendentry{$(1-\rho)\sigma^2\leq De^{\beta}\leq \sigma^2$}

\addplot [line width=1pt, color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
0	inf\\
0.01	4.4613291497622\\
0.02	3.76818196920226\\
0.03	3.36271686109409\\
0.04	3.07503478864231\\
0.05	2.8518912373281\\
0.06	2.66956968053415\\
0.07	2.51541900070689\\
0.08	2.38188760808237\\
0.09	2.26410457242598\\
0.1	2.15874405676816\\
0.11	2.06343387696383\\
0.12	1.9764224999742\\
0.13	1.89637979230066\\
0.14	1.82227182014694\\
0.15	1.75327894865999\\
0.16	1.68874042752242\\
0.17	1.62811580570598\\
0.18	1.57095739186604\\
0.19	1.51689017059576\\
0.2	1.46559687620821\\
0.21	1.41680671203878\\
0.22	1.37028669640389\\
0.23	1.32583493383305\\
0.24	1.28327531941426\\
0.25	1.242453324894\\
0.26	1.20323261174072\\
0.27	1.16549228375787\\
0.28	1.129124639587\\
0.29	1.09403331977573\\
0.3	1.06013176810005\\
0.31	1.02734194527705\\
0.32	0.995593246962474\\
0.33	0.964821588295721\\
0.34	0.93496862514604\\
0.35	0.905981088272787\\
0.36	0.877810211306091\\
0.37	0.850411237117977\\
0.38	0.823742990035815\\
0.39	0.797767503632554\\
0.4	0.772449695648264\\
0.41	0.747757083057893\\
0.42	0.723659531478833\\
0.43	0.700129034068639\\
0.44	0.67713951584394\\
0.45	0.654666659991881\\
0.46	0.632687753273106\\
0.47	0.611181548052142\\
0.48	0.59012813885431\\
0.49	0.569508851651574\\
0.5	0.549306144334055\\
};
\addlegendentry{$0\leq De^{\beta} \leq (1-\rho)\sigma^2$}
\end{axis}
\end{tikzpicture}%

==> reverse_wyner.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\draw[->, line width=1pt](0,0)--(7,0);
\draw[->, line width=1pt](0,0)--(0,5);
\draw[black,thick,anchor=north] (7,0) node{$\gamma_i$};
\draw[black,thick,anchor=north] (2.5,0) node{$\frac{1}{2}\log{\frac{1}{1-\rho_2^2}}$};
\draw[black,thick,anchor=north] (5.5,0) node{$\frac{1}{2}\log{\frac{1}{1-\rho_1^2}}$};
\draw[black,thick,anchor=east] (0,5) node{$C_{\gamma_i}(X_i;Y_i)$};
\draw[black,thick,anchor=east] (0,4.5) node{$\frac{1}{2}\log{\frac{1+\rho_1}{1-\rho_1}}$};
\draw[black,thick,anchor=east] (0,2.5) node{$\frac{1}{2}\log{\frac{1+\rho_2}{1-\rho_2}}$};
\pgfplotsset{ticks=none}
\begin{axis}[%
hide y axis,
hide x axis,
width=4in,
height=3in,
xmin=0,
xmax=0.35,
ymin=0,
ymax=0.9,
xlabel={$\gamma_i$},
ylabel={$C_{\gamma_i}({\ve X}_i,{\ve Y}_i)$},
%%legend style={legend cell align=left, align=left, draw=white!15!black}
%]
legend style={at={(0.5,0.8)}, legend cell align=center, align=center, draw=white!15!black}
]
\addplot [line width=2pt, color=red, mark options={solid, red}]
  table[row sep=crcr]{%
0	0.423648930193602\\
0.001	0.378920116711136\\
0.002	0.360382293032487\\
0.003	0.346150527632742\\
0.004	0.334146570705555\\
0.005	0.323565576064149\\
0.006	0.31399484138816\\
0.007	0.305189244476188\\
0.008	0.296989101709239\\
0.009	0.289283515156126\\
0.01	0.281991754265907\\
0.011	0.275052884201756\\
0.012	0.268419572571688\\
0.013	0.262054184693401\\
0.014	0.255926211599776\\
0.015	0.250010513716581\\
0.016	0.244286084718856\\
0.017	0.238735158819242\\
0.018	0.233342551612378\\
0.019	0.228095163873824\\
0.02	0.222981601627633\\
0.021	0.217991880825337\\
0.022	0.213117194687595\\
0.023	0.208349728186905\\
0.024	0.203682508498523\\
0.025	0.199109283247478\\
0.026	0.194624420487134\\
0.027	0.190222825849036\\
0.028	0.185899873393252\\
0.029	0.181651347488228\\
0.03	0.177473393643538\\
0.031	0.173362476665716\\
0.032	0.169315344846812\\
0.033	0.165328999155646\\
0.034	0.161400666603368\\
0.035	0.15752777711229\\
0.036	0.153707943340818\\
0.037	0.14993894301555\\
0.038	0.146218703399979\\
0.039	0.142545287592305\\
0.04	0.138916882395813\\
0.041	0.135331787546734\\
0.042	0.131788406118438\\
0.043	0.128285235948698\\
0.044	0.124820861959803\\
0.045	0.121393949260468\\
0.046	0.118003236934417\\
0.047	0.114647532433933\\
0.048	0.111325706507888\\
0.049	0.108036688603284\\
0.05	0.104779462687373\\
0.051	0.101553063444304\\
0.052	0.0983565728060565\\
0.053	0.095189116782448\\
0.054	0.0920498625593095\\
0.055	0.0889380158376092\\
0.056	0.0858528183895267\\
0.057	0.0827935458102438\\
0.058	0.0797595054466386\\
0.059	0.0767500344861642\\
0.06	0.0737644981910322\\
0.061	0.0708022882644234\\
0.062	0.0678628213368645\\
0.063	0.0649455375621433\\
0.064	0.06204989931323\\
0.065	0.0591753899696365\\
0.066	0.0563215127885006\\
0.067	0.0534877898524407\\
0.068	0.0506737610878922\\
0.069	0.0478789833482461\\
0.07	0.0451030295566374\\
0.071	0.0423454879037071\\
0.072	0.0396059610960945\\
0.073	0.0368840656517918\\
0.074	0.0341794312388394\\
0.075	0.0314917000541527\\
0.076	0.0288205262395378\\
0.077	0.0261655753322186\\
0.078	0.0235265237474106\\
0.079	0.0209030582906893\\
0.08	0.018294875698085\\
0.081	0.0157016822019983\\
0.082	0.0131231931211901\\
0.083	0.0105591324732333\\
0.084	0.00800923260794173\\
0.085	0.00547323386040482\\
0.086	0.00295088422236228\\
0.087	0.000441939030749239\\
};
\addlegendentry{$C_{\gamma_2}(X_2;Y_2)$}


\addplot [line width=2pt, color=blue , mark options={solid, blue}]
  table[row sep=crcr]{%
0	0.693147180559945\\
0.001	0.64841836707748\\
0.002	0.629880543398831\\
0.003	0.615648777999085\\
0.004	0.603644821071899\\
0.005	0.593063826430492\\
0.006	0.583493091754503\\
0.007	0.574687494842531\\
0.008	0.566487352075582\\
0.009	0.55878176552247\\
0.01	0.55149000463225\\
0.011	0.5445511345681\\
0.012	0.537917822938031\\
0.013	0.531552435059744\\
0.014	0.525424461966119\\
0.015	0.519508764082925\\
0.016	0.5137843350852\\
0.017	0.508233409185585\\
0.018	0.502840801978722\\
0.019	0.497593414240167\\
0.02	0.492479851993976\\
0.021	0.48749013119168\\
0.022	0.482615445053938\\
0.023	0.477847978553248\\
0.024	0.473180758864866\\
0.025	0.468607533613821\\
0.026	0.464122670853477\\
0.027	0.459721076215379\\
0.028	0.455398123759595\\
0.029	0.451149597854572\\
0.03	0.446971644009881\\
0.031	0.44286072703206\\
0.032	0.438813595213156\\
0.033	0.43482724952199\\
0.034	0.430898916969712\\
0.035	0.427026027478633\\
0.036	0.423206193707161\\
0.037	0.419437193381894\\
0.038	0.415716953766322\\
0.039	0.412043537958648\\
0.04	0.408415132762157\\
0.041	0.404830037913077\\
0.042	0.401286656484781\\
0.043	0.397783486315041\\
0.044	0.394319112326147\\
0.045	0.390892199626812\\
0.046	0.38750148730076\\
0.047	0.384145782800276\\
0.048	0.380823956874232\\
0.049	0.377534938969627\\
0.05	0.374277713053717\\
0.051	0.371051313810648\\
0.052	0.3678548231724\\
0.053	0.364687367148791\\
0.054	0.361548112925653\\
0.055	0.358436266203953\\
0.056	0.35535106875587\\
0.057	0.352291796176587\\
0.058	0.349257755812982\\
0.059	0.346248284852508\\
0.06	0.343262748557376\\
0.061	0.340300538630767\\
0.062	0.337361071703208\\
0.063	0.334443787928487\\
0.064	0.331548149679573\\
0.065	0.32867364033598\\
0.066	0.325819763154844\\
0.067	0.322986040218784\\
0.068	0.320172011454236\\
0.069	0.31737723371459\\
0.07	0.314601279922981\\
0.071	0.311843738270051\\
0.072	0.309104211462438\\
0.073	0.306382316018135\\
0.074	0.303677681605183\\
0.075	0.300989950420496\\
0.076	0.298318776605881\\
0.077	0.295663825698562\\
0.078	0.293024774113754\\
0.079	0.290401308657033\\
0.08	0.287793126064428\\
0.081	0.285199932568342\\
0.082	0.282621443487534\\
0.083	0.280057382839577\\
0.084	0.277507482974285\\
0.085	0.274971484226748\\
0.086	0.272449134588706\\
0.087	0.269940189397093\\
0.088	0.267444411038669\\
0.089	0.264961568669733\\
0.09	0.262491437949988\\
0.091	0.260033800789694\\
0.092	0.257588445109313\\
0.093	0.255155164610888\\
0.094	0.252733758560482\\
0.095	0.250324031581008\\
0.096	0.24792579345487\\
0.097	0.245538858935842\\
0.098	0.243163047569666\\
0.099	0.240798183522877\\
0.1	0.23844409541941\\
0.101	0.236100616184537\\
0.102	0.233767582895768\\
0.103	0.231444836640317\\
0.104	0.229132222378785\\
0.105	0.226829588814748\\
0.106	0.224536788269923\\
0.107	0.222253676564626\\
0.108	0.21998011290327\\
0.109	0.217715959764609\\
0.11	0.21546108279653\\
0.111	0.213215350715135\\
0.112	0.210978635207916\\
0.113	0.208750810840821\\
0.114	0.206531754969012\\
0.115	0.204321347651153\\
0.116	0.202119471567046\\
0.117	0.199926011938457\\
0.118	0.197740856452999\\
0.119	0.1955638951909\\
0.12	0.193395020554557\\
0.121	0.191234127200714\\
0.122	0.189081111975179\\
0.123	0.186935873849933\\
0.124	0.184798313862552\\
0.125	0.182668335057818\\
0.126	0.18054584243144\\
0.127	0.178430742875776\\
0.128	0.176322945127486\\
0.129	0.174222359717025\\
0.13	0.172128898919889\\
0.131	0.170042476709561\\
0.132	0.167963008712066\\
0.133	0.165890412162074\\
0.134	0.163824605860499\\
0.135	0.161765510133508\\
0.136	0.15971304679291\\
0.137	0.157667139097844\\
0.138	0.155627711717736\\
0.139	0.153594690696459\\
0.14	0.151568003417652\\
0.141	0.149547578571161\\
0.142	0.147533346120545\\
0.143	0.145525237271614\\
0.144	0.14352318444196\\
0.145	0.141527121231438\\
0.146	0.139536982393564\\
0.147	0.137552703807793\\
0.148	0.135574222452654\\
0.149	0.133601476379693\\
0.15	0.131634404688207\\
0.151	0.129672947500738\\
0.152	0.127717045939297\\
0.153	0.125766642102291\\
0.154	0.12382167904213\\
0.155	0.12188210074349\\
0.156	0.119947852102205\\
0.157	0.11801887890477\\
0.158	0.116095127808435\\
0.159	0.11417654632186\\
0.16	0.112263082786319\\
0.161	0.110354686357443\\
0.162	0.108451306987459\\
0.163	0.106552895407934\\
0.164	0.104659403112989\\
0.165	0.102770782342981\\
0.166	0.100886986068621\\
0.167	0.0990079679755332\\
0.168	0.0971336824492247\\
0.169	0.0952640845604573\\
0.17	0.0933991300510144\\
0.171	0.0915387753198397\\
0.172	0.0896829774095456\\
0.173	0.0878316939932715\\
0.174	0.0859848833618863\\
0.175	0.0841425044115222\\
0.176	0.0823045166314281\\
0.177	0.0804708800921363\\
0.178	0.0786415554339273\\
0.179	0.0768165038555898\\
0.18	0.0749956871034619\\
0.181	0.073179067460747\\
0.182	0.0713666077370948\\
0.183	0.0695582712584429\\
0.184	0.0677540218571057\\
0.185	0.0659538238621066\\
0.186	0.0641576420897478\\
0.187	0.0623654418344066\\
0.188	0.0605771888595535\\
0.189	0.0587928493889864\\
0.19	0.0570123900982736\\
0.191	0.0552357781064007\\
0.192	0.053462980967612\\
0.193	0.0516939666634465\\
0.194	0.0499287035949582\\
0.195	0.0481671605751172\\
0.196	0.0464093068213874\\
0.197	0.0446551119484738\\
0.198	0.0429045459612362\\
0.199	0.0411575792477646\\
0.2	0.0394141825726113\\
0.201	0.0376743270701749\\
0.202	0.0359379842382339\\
0.203	0.0342051259316231\\
0.204	0.0324757243560517\\
0.205	0.0307497520620584\\
0.206	0.0290271819390974\\
0.207	0.0273079872097554\\
0.208	0.0255921414240949\\
0.209	0.0238796184541195\\
0.21	0.0221703924883572\\
0.211	0.0204644380265633\\
0.212	0.0187617298745336\\
0.213	0.0170622431390289\\
0.214	0.0153659532228078\\
0.215	0.0136728358197622\\
0.216	0.0119828669101568\\
0.217	0.0102960227559675\\
0.218	0.00861227989631552\\
0.219	0.00693161514299756\\
0.22	0.00525400557610645\\
0.221	0.00357942853974358\\
0.222	0.00190786163781709\\
0.223	0.000239282729925572\\
};
\addlegendentry{$C_{\gamma_1}(X_1;Y_1)$}

\addplot [line width=2pt, color=black, mark options={solid, red}]
  table[row sep=crcr]{%
0.25	0\\
0.25	0.75\\
};
\addlegendentry{$\theta-$ level}

\draw[->, line width=1.5pt](0.25,0.4)--(0.2,0.4);

\end{axis}
\end{tikzpicture}%
